Reconciling Predictive and Statistical Parity: A Causal Approach

Since the rise of fair machine learning as a critical field of inquiry, many different notions on how to quantify and measure discrimination have been proposed in the literature. Some of these notions, however, were shown to be mutually incompatible. Such findings make it appear that numerous different kinds of fairness exist, thereby making a consensus on the appropriate measure of fairness harder to reach, hindering the applications of these tools in practice. In this paper, we investigate one of these key impossibility results that relates the notions of statistical and predictive parity. Specifically, we derive a new causal decomposition formula for the fairness measures associated with predictive parity, and obtain a novel insight into how this criterion is related to statistical parity through the legal doctrines of disparate treatment, disparate impact, and the notion of business necessity. Our results show that through a more careful causal analysis, the notions of statistical and predictive parity are not really mutually exclusive, but complementary and spanning a spectrum of fairness notions through the concept of business necessity. Finally, we demonstrate the importance of our findings on a real-world example.

==> sections/B-CoverLetter.tex <==
Dear AAAI Program Committee,
\vspace{0.1in}

\noindent In this cover letter, we describe the key changes that were introduced to our manuscript since its submission to NeurIPS 2023. To place these changes in context, we begin by quoting the decision of the NeurIPS meta-reviewer, after which we highlight how the comments were addressed.

\vspace{0.1in}
\begin{myquote}
\textit{Overview of Reviews:}
Reviewers engaged with this submission, highlighting several key strengths, particularly concerning its scope and technical contributions, such as the decomposition formula. After considering the rebuttal and the discussion, the reviewer recommendations ranged between "weak reject" and "weak accept." Notably, even the more positive reviewers hesitated to strongly champion the paper's acceptance. Given the borderline scores and the potential impact of this submission, I also reviewed the manuscript, taking into account the reviews, responses, and the original paper. \\

\textit{Recommendation:}
My recommendation is to reject the paper at this time given the borderline assessment by reviewers and the lack of strong support. Central to my decision is the unanimous agreement among all four reviewers that the paper would benefit from addressing several concrete suggestions. Beyond the issues pinpointed by reviewers, I urge the authors to tackle the following: \\

\textbf{(1) Business Necessity:} One novel idea introduced in the paper is "business necessity." The notion is currently used to describe one of the terms in the proposed decomposition. The paper would greatly benefit if the treatment and discussion of this notion were developed in a way that could highlight its value in practice.

\textbf{(2) Positioning in Relation to Prior Work:} Numerous reviewers voiced concerns about potential overlaps with previous works, notably those by Coston et al. 2020, Zhang and Bareinboim, Makar and D'Amour, and Nabi and Shpitser. The subsequent exchanges between reviewers and authors during the rebuttal phase further underscore the need for a more transparent and compelling delineation of these overlaps. To address this, I recommend that the authors include a lucid discussion, possibly introducing a fresh framing to distinguish their contributions from preceding research.
\end{myquote}

As can be seen, the meta-reviewer raises two key issues. The first is related to highlighting the concept of business necessity. To address this, we have adapted our submission to highlight practically how business necessity considerations can be taken into account. In particular, we now emphasize the importance of this concept in the introduction; furthermore, we also extend the discussion of this concept after introducing Algorithm 1 that represents a practical approach for incorporating considerations of business necessity.

Furthermore, the meta-reviewer also raises concerns about the clarity of relation to previous literature. To this end, we add a new section in the introduction, called ``Relationship to Previous Literature'', in which we discuss all of the related works, and clearly draw connections with them. 

We also addressed the remaining reviewer comments on (i) extending and updating the experimental results; (ii) discussing the distinction between binary vs. continuous predictors (we added Appendix D); (iii) discussing if there always exists a predictor satisfying the desired notion of fairness (Appendix E).

Therefore, we believe that we have addressed all the key concerns raised during the NeurIPS review process. 
We are looking forward to the review process at AAAI 2024, and look forward to receiving further reviewer comments.
\vspace{0.1in}

\noindent Best wishes, \\
Authors of AAAI Paper 14014

==> sections/C-ReviewResponse.tex <==
%\noindent \textbf{Review Response -- Paper 14014:}
\newcommand{\hlr}[1]{\underline{#1}}
\noindent We thank the reviewers for the time and effort in reviewing our paper. We index all weaknesses with W, questions Q, and comments C. We do not fully cite reviewer's questions (due to space limit), but provide a caption for each W/Q/C.

\subsubsection{Reviewer \#1}

[\hlr{W1: Single Dataset Evaluation}] We thank the reviewer for raising this point. Firstly, we wish to mention that further experimental results related to some of the theoretical findings can be found in Appendix A.2. Secondly, we concur with the reviewer and suggest adding another dataset, namely Census 2018. The application of Algorithm~\ref{algo:sp-to-pp-bn} on this dataset is presented in Figure 1. As for the COMPAS dataset, we see how unbiased predictors can inherit undesired bias, while causally fair predictors can satisfy the conditions of Algorithm 2. We hope this addresses the reviewer's concern.

[\hlr{W2: Discussion of Limitations}] We mention the brief discussion of limitations in the last paragraph on page 5 (regarding complexity for larger graphs). We believe there are two key possible limitations of our approach. Firstly, for the current version of Algorithm 2, the standard fairness model needs to be satisfied (although a partial identification approach is possible under additional confounding, we acknowledge this solution is not fully worked out in the current version of the paper). Secondly, when moving to more general causal diagrams (beyond the SFM), the approach scales unfavorably in the number of causal pathways. The latter limitation, however, holds for any type of causal analysis.

[\hlr{C1: Abbreviations}] Thanks a lot for pointing this out. Indeed, the paper uses multiple abbreviations. We now made sure these are introduced properly, and are emphasized in text. 
% In particular:
% %\begin{itemize}
%     %\item 
%     BN first appearance in page 1, paragraph 3, we state (labeled BN from now on),
%     %\item 
%     PP \& SP first appearance page 3, start of Section 2.1 -> we add that statistical parity (labeled SP from now on) and predictive parity (labeled PP).
%     %\item 
%     SPM first appearance in Definition 2, we now re-write: ``The predictor $\widehat{Y}$ satisfies statistical parity (SP) with respect to $X$ if $X \ci \widehat{Y}$, or equivalently if the statistical parity measure (SPM, for short) satisfies:''
% %\end{itemize}
% These changes ensure that each abbreviation is properly defined in the first appearance of the term. We thank the reviewer for this suggestion!
%
[\hlr{C2: Works cited in brackets}] Thanks; indeed, this is a mistake on our side. We have now properly bracketed this citation.
[\hlr{C3: Colors in Figure 5}] Thanks for spotting this issue as well, the text and the color scheme are indeed no longer compatible. This is now resolved!
[\hlr{C4: Figure 6 x-axis label}] Thanks, we have also implemented this suggestion.
[\hlr{C5: SP/PP swapped in Conclusion}] We thank the reviewer for spotting this issue and have updated the manuscript accordingly.
%are very glad the reviewer spotted this typo, as it clearly shows the reviewer understood the key message of the manuscript! Many thanks for this catch.
[\hlr{Q1: Single Dataset}] See response [W1] and Fig 1. [Q2: Limitations] See resp. [W2].


\subsubsection{Reviewer \#2} 
%We thank the reviewer for the time and effort spent in assessing our work. 
Since we believe there are some misconceptions about our work, especially regarding the technical soundness of the results, we respectfully ask the reviewer to reconsider it in the light of the clarifications provided below. 


[\hlr{W1: Theorem 1 Terms}] In the statement of Theorem 1, we remark that the assumed causal diagram comes from Figure 3 (with $Z = \emptyset$), please see the last sentence on page 4:
``Let $\mathcal{M}$ be an SCM compatible with the causal graph in Fig.3''.
In other words, the framing of the theorem does not consider Figure 2. Thus, there are indeed no back-door paths, and the reasoning presented is valid. We believe this should address the main concern of the reviewer.
Furthermore, in footnote 3 on page 4, we state that: 
``We remark that the essence of the argument is unchanged in the case with $Z \neq \emptyset$, but handling this case limits the clarity of presentation.''
This remark also stresses the point that Theorem 1 considers the case $Z = \emptyset$. For Z non-empty, a very similar decomposition can be obtained (in which case Term III does not vanish), but the analysis is more involved, but not more insightful for motivating the subsequent developments. We hope this clarifies the current misunderstanding. 

\begin{figure}
    \centering
    \includegraphics[width=0.7 \linewidth]{figures/census-algorithm-1.png}
    \caption*{Figure 1: Census 2018 and Algorithm~\ref{algo:sp-to-pp-bn}.}
    \label{fig:census-algo-1}
    \vspace{-0.25in}
\end{figure}


Finally, we agree with the suggestion for providing a more formal assessment of counterfactual independences. We have added an explicit derivation of the required independence, using twin networks, and added it into Appendix A.1 (proof of Thm. 1). Thank you for the suggestion.
%We thank the reviewer for this suggestion, which improves clarity. 

[\hlr{W2: Connection of Decomposition and Theorem 1}] 
We appreciate you raising this issue and we will reconstruct the argument in the sequence (step by step) to clarify the importance of the mentioned connection.

%. We wonder if our current articulation is well-phrased since we hoped this connection would come across as transparent.

%We reconstruct the argument step by step, to clarify the importance of the mentioned connection. 
\noindent \textbf{(Step 1)} We first showed that PPM = Term I + Term II. Assuming the decision-maker wants to ascertain PPM = 0, so Term I + Term II = 0, which means that  
%in other words, one must have that 
Term II = - Term I.\\
\textbf{(Step 2)} Now, Term I measures the effect of $X$ on $Y$ for a selected group of units. Even though we can select these units, we cannot control the corresponding effect measure, since $Y$ cannot be manipulated. The mechanism of $Y$ is a property of the real world, and the causal effect is not in our control. 
For concreteness, suppose that $X$ has a positive effect on $Y$ for all units $u$. Then, in whichever way units are selected, Term I will never be equal to 0 (i.e., it will be positive). Therefore, to have PPM = 0, the decision-maker needs to set Term II appropriately, to compensate that. \\ 
\textbf{(Step 3)} To achieve that Term II = - Term I, the decision-maker needs to set the causal effect of $X$ to $\widehat{Y}$ to be exactly equal to the effect of $X$ on $Y$. This exact intuition, carried over to a causal setting (i.e., focusing more granularly on direct, indirect, and spurious), underpins Def. 5 and Alg. 1.

[\hlr{W3: Direct connection \& Computing Ctf-{DE,IE,SE}}]: Here, we were surprised that the reviewer sees our approach as simply computing existing Ctf-{DE,IE,SE} measures. In particular, we believe the following are key distinctions, and important steps compared to the previous literature:
(i) Our approach considers both the true outcome $Y$ and the predictor $\widehat{Y}$, and successfully incorporates both of them in a single framework. There are almost no previous works that address this issue explicitly.
(ii)  Secondly, a typical approach of path-specific causal fairness (such as Chiappa, 2019, or Nabi \& Shpitser, 2018) would only compute Ctf-{DE, IE, SE} for pathways \textit{that are discriminatory}. That is, pathways in the business necessity set are not considered in the analysis. Furthermore, for BN paths, the condition Ctf-CE(y) = Ctf-CE($\widehat{y}$) is not even tested. Thus, our approach is the first to integrate business necessity considerations (and show how they bridge the gap between SP and PP), filling a major gap in the current literature.

% [Q1: Back-door paths] Please see response [W1]. 
% [Q2: Connection of PP decomposition and CPP] Please see responses [W2]+[W3]. 


==> sections/D-MessageToAC.tex <==
\newpage

\subsection*{Message to the AC}

Dear Area Chair,

\noindent We would like to respectfully call your attention to the review we received from Reviewer \#2. Unfortunately, we are unsure if this reviewer assessed our paper adequately. In particular, the reviewer writes that:
"the proof [of Theoorem 1] states that there are no backdoor paths between X and $Y,\hat{Y}$. This is confusing as there are backdoor paths $X <--> Z -->Y$."
However, in the theorem statement, we explicitly point to a figure of a causal diagram which does not have the $Z$ variable. Quoting directly from the paper:
"Let $\mathcal{M}$ be an SCM compatible with the causal graph in Fig. 3."
When checking Fig. 3, one can immediately see there is no $Z$ in the graph. Furthermore, in an explicit remark in the footnote, we even say:
"We remark that the essence of the argument is unchanged in the case with $Z \neq \emptyset$, but handling this case limits the clarity of presentation."
Therefore, the text could hardly make it more clear that the graph has no $Z$ variables, which brings into question how this could have possibly been missed by the reviewer. Furthermore, this also seems to constitute the reviewer's main concern, and based on this misconception, the reviewer concludes that the claims in our paper are not presented convincingly, and gives a negative review.

Since we obtained only two reviews, we are respectfully hoping that the Area Chair may take into consideration that one of the reviews may be inadequate and try to calibrate accordingly. 
For context, it should be noted that among the five reviews we obtained for NeurIPS, none expressed concerns similar to those of Reviewer \#2; all reviewers assessed our results to be sound. The main concerns in previous reviews related to a clear connection to existing literature, which we have thoroughly addressed in this iteration of the manuscript, as elaborated in the cover letter.

\noindent We appreciate in advance your help and care, thank you, \\ 
Authors of paper \#14014
